The Lyman-alpha Emission Line as a Cosmological Tool

This thesis deals with different aspects of a special kind of high redshift galaxy, namely Ly-alpha emitters. Ly-alpha emitters are galaxies found through their Ly-alpha emission, at redshifts larger than z >~ 2 where the emission line has been redshifted into the optical or near-infrared regime. The thesis has two main parts; a lower redshift, observational part (z ~ 3) and a more technical/theoretical very high redshift part (z ~ 9). In the first, lower redshift part I present the analysis of a narrow-band image taken in the GOODS-S field, focused on a redshift for Ly-alpha of z = 3.15. The image, covering a central part of the GOODS-S field revealed 25 Ly-alpha emitting candidates, of which one turned out to be a so-called Ly-alpha blob. In the second part, I discuss future, very high redshift narrow-band surveys for Ly-alpha emitters. Finally, in a project unrelated to the other two parts of the thesis, I present a search for a 'Fundamental plane' of Ly-alpha emitters in the colour space produced by large-scale multi-wavelength surveys such as GOODS or COSMOS. [Abridged]

==> CHAPTER5/predictions.tex <==
\chapter{Predicting results from very high redshift Ly$\alpha$ surveys}\label{chapter:predictions}
\markboth{Chapter 5}{Very high redshift Ly$\alpha$ emitters}
This paper has been accepted for publication in 
\emph{Astronomy \& Astrophysics} on August
2007. The authors are Nilsson, K.K., Orsi, A., Lacey, C.G., Baugh, C.M., \& Thommes, E.

\section{Abstract}
\emph{Context} Many current and future surveys aim to detect the highest 
redshift
($z \gtrsim 7$) sources through their Lyman-{\ly} (Ly$\alpha$) emission,
using the narrow-band imaging method. However, to date the surveys have only
yielded non-detections and upper limits as no survey has reached the necessary
combination of depth and area to detect these first star forming galaxies.

\noindent \emph{Aims} On the background of observations of Ly$\alpha$-emitters at 
redshifts
$z = 5 - 7$, we aim to optimise current and future surveys for very high
redshift Ly$\alpha$-emitters by calculating model luminosity functions.
In this frame-work, we also make specific predictions for
future surveys, using various theoretical models as well as comparing results
at lower redshifts.

\noindent \emph{Methods} We combine results from several different models. We compute 
luminosity functions
at several redshifts, using a semi-analytical model and1 a simple
phenomenological model. The results are compared with observations
made at redshifts $z \sim 5.7$ and $z \sim 6.5$, and the models are then
extrapolated to higher redshift.

\noindent \emph{Results} We present luminosity functions for redshifts between 
$z = 7 - 12.5$ and
give specific number predictions for future planned or possible narrow-band
surveys for Ly$\alpha$-emitters. We also study the possibility of
constraining the very high redshift Ly$\alpha$ luminosity function with
future observations.

\noindent \emph{Conclusion} It is possible to observe $z = 7 - 10$ Ly$\alpha$-emitters 
with present, or
near-future instruments if enough observing time is dedicated. In particular
large area surveys such as ELVIS (Emission Line galaxies with VISTA Survey)
will be useful in collecting a large sample. However,
to get a large enough sample to well constrain the very high redshift
luminosity function, instruments further in the future, such as an ELT, will be
necessary.

\section{Introduction}
One of the most promising ways of detecting very high redshift ($z \gtrsim 5$),
star-forming galaxies is via narrow-band imaging surveys targeting 
Lyman-$\alpha$ (Ly$\alpha$). 
The reason for why narrow-band 
surveys are restricted to a discrete number of redshifts is the night sky
OH emission lines. According to the OH line atlas of Rousselot et al. (2000),
at Ly$\alpha$ redshifts $z_{Ly\alpha} \gtrsim 7$ ($\lambda \gtrsim 9800$~{\AA})
there are only a few possible wavelengths where a narrow-band filter can
fit in between the OH sky lines. These correspond to
$z_{Ly\alpha} \approx 7.7$,~$8.2$,~$8.8$,~$9.4$ and $10.1 - 10.5$. Several
future surveys will target these windows in the sky aiming to detect very high
redshift galaxies and several groups have already conducted narrow-band surveys
for Ly$\alpha$ at,
in particular, redshifts $z \sim 5.7$~and~$6.5$ (e.g. Ajiki et al. 2003;
Hu et al. 2004; Shimasaku et al. 2005; Ouchi et al. 2005; Malhotra et
al. 2005; Taniguchi et al. 2005; Tapken et al. 2006; Kashikawa et al. 2006).
The current redshift record for a spectroscopically confirmed Ly$\alpha$-emitter
(LEGO; see M{\o}ller \& Fynbo 2001)
is $z = 6.96$ (Iye et al. 2006) although Stark et al. (2007) have suggested
the discovery of two Ly$\alpha$-emitters at $z = 8.99$~and~$9.32$.
Three completed narrow-band surveys for Ly$\alpha$ at
redshift $z \sim 8.8$ have been presented (Parkes, Collins \& Joseph 1994;
Willis \& Courbin 2005; Cuby et
al. 2007) but have only yielded upper limits. Two future surveys have also been
presented; DaZle (Dark Ages Z Lyman-$\alpha$ Explorer, Horton et al. 2004) and
ELVIS (Emission-Line galaxies with VISTA Survey, Nilsson et al. 2006b).

During the last years, some progress in theoretical work on
Ly$\alpha$ emitting galaxies has been made.
Haiman \& Spaans (1999) have made predictions of the number counts of galaxies
linking
Ly$\alpha$ emission to halo mass. Barton et al. (2004) and Furlanetto et al.
(2005) used gas-dynamical simulations to calculate Ly$\alpha$ emission in
star forming galaxies. More
recently, Laursen \& Sommer-Larsen (2007) made predictions of the surface
brightness of galaxies based on a Ly$\alpha$ radiative transfer code applied
to an N-body/hydrodynamical simulation. In particular, two
models have been shown to be successful in reproducing the number counts of
Ly$\alpha$ emitting galaxies at high redshifts; first, the phenomenological
model of Thommes \& Meisenheimer (2005; see also Stark, Loeb \& Ellis 2007),
which is used to calculate the
expected number density of Ly$\alpha$ galaxies, and secondly the
semi-analytical
model GALFORM detailed in Le Delliou et al. (2005, 2006), which has been
successful in reproducing the luminosity functions of Ly$\alpha$ emitting
galaxies in the range $3<z<6$ and also the clustering
(Orsi et al., in prep.).

In this paper we aim to optimise future
planned, or conceivable, narrow-band surveys for very high redshift LEGOs.
We make predictions based on two approaches; a phenomenological
and a semi-analytical.
In section~\ref{sec:models} we present the different models used to make the
predictions and in section~\ref{sec:lf} we present the expected number counts
and comparisons with observed luminosity functions at lower redshift.
In section~\ref{sec:future} we make specific number predictions for some future
surveys. The conclusion is found in section~\ref{sec:conclusion}.

\vskip 5mm
Throughout this paper, we assume a cosmology with $H_0=70$
km s$^{-1}$ Mpc$^{-1}$, $\Omega _{\rm m}=0.3$ and $\Omega _\Lambda=0.7$.

\section{Models}\label{sec:models}
We use two theoretical models for high redshift
Ly$\alpha$-emitters. The first model is based on semi-analytical simulations 
(Le Delliou et al. 2005, 2006; Orsi et al., in prep.), and the second is based 
on a phenomenological approach as
presented by Thommes \& Meisenheimer (2005).

\subsection{Semi-analytical model}
The semi-analytical model GALFORM (Cole et al. 2000; Baugh et al. 2005) has 
been shown to be successful in reproducing the high redshift Universe in the 
range 
$z = 3 - 6$ (Le Delliou et al. 2005; 2006). The semi-analytical approach 
allows us to obtain the properties of the Ly$\alpha$ emission of galaxies and
their abundances as a function of redshift, calculating the star formation
histories for the entire galaxy population, following a hierarchical evolution
of the galaxy host haloes. In addition, when incorporated into an N-body
simulation, we also obtain spatial clustering information. This model has been
incorporated into the largest N-body simulation to date, the Millennium
Simulation (Springel et al., 2005), to predict clustering
properties of Ly$\alpha$ galaxies. These results will be presented in a
forthcoming paper (Orsi et al., in prep.).

The semi-analytical model assumes a top-heavy
IMF for starbursts, and a Kennicutt IMF for quiescent galaxies. The amount of
Ly$\alpha$ flux which escapes from the galaxy is modelled by a constant escape
fraction $f_{esc} = 0.02$, regardless of galaxy dust properties. It assumes a
redshift of reionisation $z_{reio} = 10$.

\subsection{Phenomenological model}
The model presented by Thommes and Meisenheimer (2005; TM05 hereafter)
allows us to calculate the expected number density of Ly$\alpha$ emitters for 
a given redshift. The model computes the evolution of the Ly$\alpha$ 
luminosity as a function of time, galaxy mass and the galaxy formation
history. The time evolution of the Ly$\alpha$ luminosity is described with a
Gaussian with a fixed FWHM, which gives the duration of the Ly$\alpha$ bright
phase. Furthermore, the SFR and the maximum Ly$\alpha$ luminosity are
assumed to be
proportional to the baryonic mass of the galaxy, and inversely proportional to
$1/t_s$, where $t_s$ is the collapse time of gas inside haloes. The model also
computes the
fraction of galaxies for a given mass and redshift with current Ly$\alpha$
emission, $P_M(t)$, and so the number density of galaxies at redshift $z_0$
with baryonic mass $M$ and ignition time $t_i$, where $t_i < t(z_0)$, is
$\Phi(M,0)P_M(t_i)$. The total number of galaxies is obtained by integrating
over a range of masses and ignition times characterized by $z_0$ and some free
parameters, fixed to match the number counts of galaxies at $3.5<z<5.7$. In
this sense, the TM05 model uses a similar approach to semi-analytic modelling
to adjust the free parameters.

\section{Number counts}\label{sec:lf}
The possible Ly$\alpha$ redshifts between redshift $z = 7 - 10$ where a 
narrow-band filter can be placed are 
$z_{Ly\alpha} = 7.7, 8.2, 8.8,$~and~$9.4$. Redshifts beyond 10 are unreachable with
the ground-based instruments of the near-future. However, one possibility for
these redshift larger than 10 surveys may be the James Webb Space Telescope (JWST,
see section~\ref{subsec:jwst}) and hence we choose to make predictions also for redshift 
$z_{Ly\alpha} = 12.5$.
First, we wish to compare the number counts from different methods. In
Fig.~\ref{fig:oldplot}, we plot the expected cumulative Ly$\alpha$ luminosity function
for redshifts
5.7 and 6.5 from the semi-analytical model and the phenomenological model, and the
observed luminosity functions of several published surveys.
\begin{figure}[!t]
\begin{center}
\epsfig{file=CHAPTER5/plot1.ps,width=11.0cm}
\caption[Luminosity functions at redshift $z = 5.7$ and $z = 6.5$]{Plot of luminosity functions at redshifts $z = 5.7$ and $6.5$. Red  
points and lines are at redshift $z = 5.7$, black points/lines at redshift
$z = 6.5$. Points are observations by Ajiki et al. (2003; redshift 5.7,
squares), Hu et al. (2004; redshift 5.7, pluses), Taniguchi et al. (2005;
redshift 6.5, crosses), Shimasaku et al. (2006; redshift 5.7,
diamonds), Kashikawa et al. (2006; redshift 6.5, stars) and
Malhotra \& Rhoads (2004; redshift 5.7 and 6.5, triangles). Solid lines mark
semi-analytic models, dot-dashed lines the Thommes \& Meisenheimer (2005)
models.}
\label{fig:oldplot}
\end{center}
\end{figure}
We can see that the models match the observed data. The error bars on the data
points, omitted in the plot in order to not confuse the points, are large; in
the bright end of the luminosity function due to small number statistics and in
the faint end due to incompleteness in the samples. The semi-analytic model tends
to under-estimate the redshift $z = 6.5$ luminosity function, but fits the
$z = 5.7$ luminosity function well. The TM05 model has the opposite appearance,
i.e. it fits the $z = 6.5$ luminosity function well, but under-estimates the
$z = 5.7$ luminosity function. Overall, the two models match the data well and
hence we conclude that these models can be used to extrapolate to higher
redshifts.

There are now several ways of extrapolating to higher redshifts.
Firstly, we can immediately calculate the expected luminosity functions at any
redshift from the two models. This gives two predictions per redshift. A third
method would be to extrapolate the parameters of Schechter functions fitted to
the lower redshift, observed data. The Schechter function describes
a luminosity function and has the following form
\begin{equation}
\phi(L)dL = \phi^{\star}(L/L^{\star})^{\alpha}\mathrm{exp}(-L/L^{\star})dL/L^{\star}
\end{equation}
where the shape of the function is determined by the three parameters $\alpha$,
$\phi^{\star}$ and $L^{\star}$. For our extrapolation, we use fits to
observations at redshift $z \approx 3$
(van Breukelen et al. 2005; Gronwall et al. 2007),
$z \approx 5.7$
(Malhotra \& Rhoads 2004; Shimasaku et al. 2006) and $z \approx 6.5$
(Malhotra \& Rhoads 2004; Kashikawa et al. 2006). For simplicity, we assume a faint
end slope of $\alpha = 1.5$, and the values used in the extrapolation are shown
in Table~\ref{tab:lfdata}.
\begin{table}[!t]
\begin{center}
\caption[Parameters of Schechter functions found in previous publications]{Parameters of the fitted Schechter function in previously published
papers. References are 1) van Breukelen et al. (2005), 2) Gronwall et al. (2007),
3) Malhotra \& Rhoads (2004), 4) Shimasaku et al. (2006) and 5) Kashikawa et al.
(2006). The latter three references fit for three faint end slopes
($\alpha = 1.0, 1.5$~and~$2.0$), but here we only reproduce the results for
fits with $\alpha = 1.5$ as we fix the slope in our calculations. Malhotra
\& Rhoads (2004) does not give error bars on the fits.}
\vspace{0.5cm}
\begin{tabular}{lccccccccc}
\hline
\hline
Ref & Redshift & $\alpha$ & $\log{\phi^{\star} \mathrm{Mpc}^{-3}}$ & $\log{L^{\star} \mathrm{ergs/s}}$ & \\
\hline
1 & $\sim 3.2$ & $1.6$  & $-2.92^{+0.15}_{-0.23}$ & $42.70^{+0.13}_{-0.19}$ & \\
2 &       3.1  & $1.49^{+0.45}_{-0.54}$ & $-2.84$ & $42.46^{+0.26}_{-0.15}$ & \\
3 &       5.7  & $1.5$  & $-4.0$ & $43.0$ & \\
4 &       5.7  & $1.5$  & $-3.44^{+0.20}_{-0.16}$ & $43.04^{+0.12}_{-0.14}$ & \\
3 &       6.5  & $1.5$  & $-3.3$ & $42.6$ & \\
5 &       6.5  & $1.5$  & $-2.88^{+0.24}_{-0.26}$ & $42.60^{+0.12}_{-0.10}$ & \\
\hline
\label{tab:lfdata}
\end{tabular}
\end{center}
\end{table}
The values of $\phi^{\star}$ and $L^{\star}$ are then fitted with a linear fit,
as this is the simplest form of extrapolation,
and extrapolated to higher redshifts. The values we find for the higher redshifts of
interest to us can be found in Table~\ref{tab:lfnew}.
\begin{table}[!t]
\begin{center}
\caption[Extrapolated parameters of the observed Schechter function]{Extrapolated parameters of the observed Schechter function at lower
redshifts. The faint end slope is fixed to $\alpha = 1.5$.}
\vspace{0.5cm}
\begin{tabular}{lccccccccc} 
\hline
\hline
Redshift & $\log{\phi^{\star} \mathrm{Mpc}^{-3}}$ & $\log{L^{\star} \mathrm{ergs/s}}$ & \\
\hline
7.7  & $-3.82 \pm 0.74$ & $42.91 \pm 0.34$ & \\
8.2  & $-3.92 \pm 0.74$ & $42.94 \pm 0.34$ & \\
8.8  & $-4.03 \pm 0.74$ & $42.97 \pm 0.34$ & \\
9.4  & $-4.14 \pm 0.74$ & $43.01 \pm 0.34$ & \\
12.5 & $-4.73 \pm 0.74$ & $43.19 \pm 0.34$ & \\
\hline
\label{tab:lfnew}
\end{tabular}
\end{center}
\end{table}

In Fig.~\ref{fig:newplot} we now plot the expected luminosity functions, calculated
through the three methods mentioned above and for three redshifts. For
other redshifts, the curves may be interpolated.
\begin{figure}[!t]
\begin{center}
\epsfig{file=CHAPTER5/plot2.ps,width=11.0cm}
\caption[Ly$\alpha$ luminosity functions at higher redshifts]{Ly$\alpha$ luminosity functions at higher redshifts. Red lines are
extrapolations from observed luminosity functions at lower redshift, green lines are TM05 models and black lines are semi-analytical models. Different
linestyles show different redshifts. Hatched area marks upper limits from
Willis \& Courbin (2005) and Cuby et al. (2006), both at redshift $z =  8.8$.}
\label{fig:newplot}  
\end{center}\end{figure}
We can see that the predictions agree very well with each other at redshift
$z = 7.7$, and
then agree gradually worse as the redshift increases. For the highest redshift,
$z = 12.5$, TM05 fails in producing a prediction due to too small number counts.

There are several reasons for why predictions at redshift $z = 12.5$ are
difficult. Even though only $\sim 200$~Myrs separate the ages of the Universe
between redshift 8.8~and~12.5, the Universe went through an important
transition at this time as re-ionisation occurred (Spergel et al. 2007). However, we do
not know exactly how and when this happened and the number counts of
observable galaxies at redshifts above 10 are hence, today,
very poorly constrained.

In next section, we discuss more specific predictions for a few known and conceivable
future surveys.

\section{Future surveys}\label{sec:future}

\subsection{DaZle -- Dark ages \emph{z} {\ly} Explorer}
DaZle is a visitor mode instrument placed on the VLT UT3 (Horton et al. 2004).
The instrument is designed to use a narrow-band differential imaging
technique, i.e. observing the same field with two very narrow filters with
slightly offset central wavelength. Objects with Ly{\ly} in one of the filters
can then be selected from the differential image of both filters. The
field-of-view of DaZle is $6.83' \times 6.83'$ and it is expected to reach
a flux level of $2 \times 10^{-18}$~erg~s$^{-1}$~cm$^{-2}$ (5$\sigma$) in
10 hours of integration in one filter. This corresponds to a luminosity limit at
redshift $z = 7.7$ of $\log{(\mathrm{L}_{Ly\alpha})} = 42.13$~erg~s$^{-1}$.
The two initial filters are centred
on $z_{Ly\alpha} = 7.68$~and~$7.73$ and at this redshift, the surveyed
volume becomes $1336$~Mpc$^3$ per pointing per filter pair. Thus, from
Fig.~\ref{fig:newplot}, we can conclude that DaZle will discover
$\sim 0.13 - 0.37$ candidates with one pointing and filter pair.


\subsection{ELVIS -- Emission Line galaxies with VISTA Survey}
ELVIS\footnote{www.astro.ku.dk/$\sim$kim/ELVIS.html} is part of Ultra-VISTA, 
a future ESO Public Survey with  
VISTA\footnote{www.vista.ac.uk} (Visible and Infrared Survey Telescope
for Astronomy). Ultra-VISTA is planned to do very deep near-infrared broad-
and narrow-band imaging in the COSMOS field. It will observe four strips
with a total area of 0.9~deg$^2$. The narrow-band filter is focused on
the $z_{Ly\alpha} = 8.8$ sky background window with central wavelength $\lambda_c = 1185$~nm.
The flux limit of the narrow-band images is expected to reach
$3.7 \times 10^{-18}$~erg~s$^{-1}$~cm$^{-2}$ (5$\sigma$) after the full survey
has been completed. Ultra-VISTA will run from early 2008 for about 5 years and all the data will be public. ELVIS is presented further in Nilsson et al. (2006b).
ELVIS will survey several different emission-lines (e.g. H$\alpha$ at redshift
$z = 0.8$, [OIII] at redshift $z = 1.4$ and [OII] at redshift $z = 2.2$) as well 
as the Ly{\ly} line. When the survey is complete, the final mosaic will reach a 
Ly{\ly} luminosity limit of $\log{(\mathrm{L}_{Ly\alpha})} = 42.53$~erg~s$^{-1}$.
The volume surveyed will be $540 835$~Mpc$^3$. From Fig.~\ref{fig:newplot} we see
that ELVIS should be expected to detect $3 - 40$ LEGOs.

\subsubsection{Cosmic variance}
Of the surveys at these redshifts that have been presented in previous
articles (ISAAC, DaZle and ELVIS), or are conceivable (JWST, see 
section~\ref{subsec:jwst}) only ELVIS will detect a large enough sample to 
discuss potential luminosity functions and the extent of reionisation at this 
redshift. We here discuss the results of the semi-analytical modelling on this 
aspect for ELVIS. From the semi-analytical modelling, we can make mock 
observations of the ELVIS volume. The procedure to produce these catalogues is 
explained in Orsi et al. (in prep.). 

From the mock catalogues, we can make mock 
luminosity functions of Ly$\alpha$-emitters at redshift $z = 8.8$. In 
Fig.~\ref{fig:cosvar} we plot the observed luminosity function in the different 
catalogues.
\begin{figure}[!t]
\begin{center}
\epsfig{file=CHAPTER5/elvis_lf.ps,width=9.2cm}
\caption[Observed mock luminosity functions in ELVIS]{Observed mock luminosity functions in ELVIS. Open circles show binned
number count in each mock catalogue, binned in three bins. Black dot with
error bars show the median in each bin. Thin lines are best fit
Schechter functions with different faint end slopes. Thick dashed line
represents the ``true'' luminosity function, as measured in the total
Millenium Run volume.}
\label{fig:cosvar} 
\end{center}
\end{figure}
The spread in number density between the catalogues is large, and it will be
hard to make an accurate fit to the luminosity function using only the sample
from the ELVIS survey. However, if all the data is binned in one bin, it maybe 
possible to normalise the luminosity function at redshift $z = 8.8$, assuming a 
value for the slope and $L_{\star}$.

It has also been suggested that the clustering of Ly$\alpha$-sources at these
redshifts will reveal the level of ionisation (McQuinn et al. 2007). McQuinn et
al. (2007) establish that large HII bubbles may exist during reionisation,
and that these will enhance the observed clustering of Ly$\alpha$-emitters
in proportion to the fraction of neutral hydrogen in the Universe. A sample of
$\sim 50$ emitters will be enough to constrain the level of reionisation
(McQuinn, priv. communication), almost within reach of the ELVIS survey. A
future, extended version of ELVIS would be able to place very tight constraints
on re-ionisation.

\subsection{JWST}\label{subsec:jwst}
A possibility even further into the future is to use the James Webb
Space Telescope\footnote{www.jwst.nasa.gov} (JWST). JWST is scheduled
for launch in 2013 and will have excellent capabilities within the near- and
mid-infrared regions of the spectrum. Two of the instruments aboard JWST
could be used for narrow-band surveys; NIRCam, the near-infrared camera, and
TFI, the tunable filter imager (for a review on JWST see Gardner et al. 2006).
NIRCam will have 31 filters, of which nine are
narrow-band filters. The filter with shortest wavelength has central wavelength
$\lambda_c = 1.644$~$\mu$m (F164N; $z_{Ly\alpha} = 12.5$). TFI will have
tunable filters with variable central wavelength, however it is only 
sensitive at wavelengths larger than $\lambda \sim 1.6$~$\mu$m. NIRCam is 
expected to reach a flux limit of
$\sim 1 \times 10^{-18}$~erg~s$^{-1}$~cm$^{-2}$ (5$\sigma$) in $10000$~s
of exposure time. Hence, a flux limit of
$\sim 5 \times 10^{-19}$~erg~s$^{-1}$~cm$^{-2}$ (5$\sigma$, $\log{(\mathrm{L}_{Ly\alpha})} = 42.00$~erg~s$^{-1}$.) could be reached
in 10 hours, assuming that the sensitivity is proportional to the square root
of the exposure time. TFI is expected to be able to reach a flux limit almost
a factor of two deeper in the same time, however it has a field-of-view of
only half of the NIRCam (which is $2 \times 2.16' \times 2.16'$). In one
NIRCam pointing at redshift $z = 12.5$, approximately $1643$~Mpc$^3$ are 
surveyed. Again, from Fig.~\ref{fig:newplot}, we can estimate that we will detect
$\lesssim 0.1$ galaxies per 10-hour pointing with NIRCam.

\section{Discussion}\label{sec:conclusion}
Several factors enter into the error bars of our predictions. A problem is the
lack off, or disagreement between, observed lower redshift luminosity
functions. There are many caveats in producing Ly$\alpha$ luminosity functions,
of which the selection function is the most difficult to correct for.
The problem arises from that the filter transmission curve is not box-shaped,
but rather gaussian. Thus, only brighter objects will be observed at the wings
of the filter, and these will be observed to have smaller than intrinsic
luminosities. Secondly, the equivalent width (EW) limit that the survey is
complete to depends on the depth of the broad-band images used for the
selection. Thirdly, if the sample is a photometric sample, it is possible
that there are lower redshift interlopers, where the emission line is e.g. [OII], 
in the sample. Finally, the
samples are still so small that we have to deal with small number statistics.
All of these problems cause the observed luminosity function at lower
redshifts to be uncertain.

Our models also have inherent error sources. The semi-analytical model assumes a 
top-heavy IMF and a constant escape fraction of $f_{esc} = 0.02$, two
parameters determined from best fit with observed data (Le Delliou et al. 2005).
It also assumes an instantaneous re-ionisation at redshift $z = 10$, which
is unphysical. This will affect predictions at redshifts less than 10
if re-ionisation was not complete at these redshifts, by the decreasing the
actual observed number compared to the models. The science
case for many of these surveys is thus to determine the fraction of neutral
hydrogen in the Universe at these redshifts. The TM05 model fits observed
data very well but is very simplified and so there are no guarantees that
the extrapolation to higher redshifts gives accurate predictions.

We summarise the number predictions for narrow-band surveys in Fig.~\ref{fig:ngal}.
\begin{figure}[!t]
\begin{center} 
\epsfig{file=CHAPTER5/ngal_z.ps,width=9.2cm}
\caption[Summary of predictions]{Summary of predictions. Plot shows number of candidates expected
per square degree per redshift interval $\Delta z = 0.1$ as a function of
redshift and observed flux limit. Points mark already observed and future
planned/proposed surveys; observations at redshift $z = 5.7$ by
Shimasaku et al. (2006; burgundy star), upper limits at redshift $z = 8.8$
by Willis \& Courbin (2005; yellow star) and Cuby et al. (2007; blue star)
and predictions of the future surveys DaZle (green star), ELVIS (red star)
and JWST (pink star).}
\label{fig:ngal}
\end{center}
\end{figure}
It is apparent that the key to acquiring a large sample of Ly$\alpha$-emitting
galaxies at redshifts greater than 7 is both depth and area. In a recent
paper, Stark, Loeb \& Ellis (2007) suggest that one of the most efficient
means of finding very high redshift Ly$\alpha$-emitters is through
spectroscopic surveys focused on gravitational lensing clusters. Lensing
surveys could easily reach down to a luminosity limit of
$10^{40.5}$~erg~s$^{-1}$ in a few times ten hours. However, the surveyed
volumes are very small, of the order of a hundred Mpc$^3$. It is very
difficult to predict what the luminosity function at these luminosities
look like, as the faint end of the Ly$\alpha$ luminosity function is poorly
constrained at all redshifts. However, both the semi-analytical model and
the model of TM05 presented here display a drop-off in number counts in
the faint end. Presumably, lensing and narrow-band surveys are complimentary
to each other as they probe different parts of the luminosity function.
With either type of survey, reaching a significant sample of redshift
$z \sim 7 - 8$ will be possible in the next few years with
telescopes/instruments in use or soon available. To reach redshifts
$z \gtrsim 10$ in significant numbers we will probably have to await
even further future instruments. If a future 40-m ELT (Extremely Large
Telescope) would be equipped with a wide-field NIR imager and a similar
width narrow-band filter as ELVIS, it could reach a luminosity limit of
$L \sim 10^{41.2}$~erg~s$^{-1}$ at redshift $z = 10.1$ (where a suitably
large sky window exists) in approximately 20 hours. Interpolating between
the $z = 12.5$ and $z = 8.8$ lines for the semi-analytical model in
Fig.~\ref{fig:newplot}, at this luminosity limit the number density should be
N($>$L)$\approx 7 \times 10^{-4}$~Mpc$^{-3}$. Thus, to get a sample of
ten Ly$\alpha$-emitters would require an area on the sky of approximately
97~square arcminutes, within three pointings if the detector has a
field-of-view of 6~arcmin on a side, as suggested by the ESO ELT Working
Group\footnote{http://www.eso.org/projects/e-elt/Publications/ELT\_INSWG\_FINAL\_REPORT.pdf}. It should of course be noted that these are very
tentative numbers, but they display the possibilities of far future
instruments.








